A Large Scale Empirical Study of the Impact of Spaghetti Code and Blob Anti-patterns on Program Comprehension

Context: Several studies investigated the impact of anti-patterns (i.e., "poor" solutions to recurring design problems) during maintenance activities and reported that anti-patterns significantly affect the developers' effort required to edit files. However, before developers edit files, they must understand the source code of the systems. This source code must be easy to understand by developers. Objective: In this work, we provide a complete assessment of the impact of two instances of two anti-patterns, Blob or Spaghetti Code, on program comprehension. Method: We analyze the impact of these two anti-patterns through three empirical studies conducted at Polytechnique Montr\'eal (Canada) with 24 participants; at Carlton University (Canada) with 30 participants; and at University Basilicata (Italy) with 79 participants. Results: We collect data from 372 tasks obtained thanks to 133 different participants from the three universities. We use three metrics to assess the developers' comprehension of the source code: (1) the duration to complete each task; (2) their percentage of correct answers; and, (3) the NASA task load index for their effort. Conclusions: We report that, although single occurrences of Blob or Spaghetti code anti-patterns have little effect on code comprehension, two occurrences of either Blob or Spaghetti Code significantly increases the developers' time spent in their tasks, reduce their percentage of correct answers, and increase their effort. Hence, we recommend that developers act on both anti-patterns, which should be refactored out of the source code whenever possible. We also recommend further studies on combinations of anti-patterns rather than on single anti-patterns one at a time.

==> sec-abstract.tex <==
% !TeX root = text-main.tex
% !TeX spellcheck = en_US
% !TeX encoding = UTF-8%
\noindent
\textbf{Context:}
Several studies investigated the impact of anti-patterns (\textit{i.e.,} ``poor'' solutions to recurring design problems) during maintenance activities and reported that anti-patterns significantly affect the developers' effort required to edit files. However, before developers edit files, they must understand the source code of the systems. This source code must be easy to understand by developers.

\noindent
\textbf{Objective:}
In this work, we provide a complete assessment of the impact of two instances of two anti-patterns, Blob or Spaghetti Code, on program comprehension.

\noindent
\textbf{Method:}
We analyze the impact of these two anti-patterns through three empirical studies conducted at Polytechnique Montréal (Canada) with 24 participants; at Carlton University (Canada) with 30 participants; and at University Basilicata (Italy) with 79 participants.

\noindent
\textbf{Results:}
We collect data from 372 tasks obtained thanks to 133 different participants from the three universities. We use three metrics to assess the developers' comprehension of the source code: (1) the duration to complete each task; (2) their percentage of correct answers; and, (3) the NASA task load index for their effort.

\noindent
\textbf{Conclusions:}
We report that, although single occurrences of Blob or Spaghetti code anti-patterns have little effect on code comprehension, two occurrences of either Blob or Spaghetti Code significantly increases the developers' time spent in their tasks, reduce their percentage of correct answers, and increase their effort. Hence, we recommend that developers act on both anti-patterns, which should be refactored out of the source code whenever possible. We also recommend further studies on \emph{combinations} of anti-patterns rather than on single anti-patterns one at a time.


==> sec-results-blob.tex <==
% !TeX root = text-main.tex
% !TeX spellcheck = en_US
% !TeX encoding = UTF-8%
\subsection{Results of the Experiments with Blob Anti-pattern} \label{sec:results-blob}

This section presents the results of the experiments that use the Blob anti-pattern. It presents the \textit{descriptive statistics} for each one of the dependent variables together with \textit{boxplots}. Subsequently, it shows the results of the hypotheses testing.

\autoref{tab:ds-blob} reports the descriptive statistics regarding the \emph{time} spent (in seconds) during the tasks,  correctness of the \emph{answers} (in percentage), and the \emph{effort} (in percentage) used to complete the tasks.
The tasks performed  on code containing the anti-pattern Blob are, on average, \emph{33.85\% more time consuming} when compared to code without the anti-pattern.
The answers in the tasks containing the anti-pattern Blob is, on average, \emph{22.07\% less accurate} when compared to task with code without the anti-pattern.
Finally, the participants, on average, reported using \emph{more effort (around 10\% more)} when performing tasks involving code that contained the anti-pattern Blob.

\begin{table}
\footnotesize
\caption{Descriptive statistics showing the aggregated results for the anti-pattern \emph{Blob}.}
\label{tab:ds-blob}
\centering
\begin{tabular*}{\tblwidth}{@{}Llrrrrr@{}}
\toprule
D.Var. & Treat. & \multicolumn{1}{l}{Mean} & \multicolumn{1}{l}{Median} & \multicolumn{1}{l}{SD} & \multicolumn{1}{l}{Min} & \multicolumn{1}{l}{Max} \\ \midrule
Time & - & 155.14 & 153.17 & 60.05 & 38.25 & 319.67 \\
Time & Blob & 234.55 & 234.92 & 81.58 & 87.58 & 434.17 \\  \addlinespace
Answer & - & 60.37 & 56.17 & 18.09 & 25.00 & 95.83 \\
Answer & Blob & 38.30 & 37.33 & 18.02 & 5.50 & 71.00 \\  \addlinespace
Effort & - & 52.61 & 52.17 & 10.88 & 34.17 & 75.75 \\
Effort & Blob & 62.47 & 63.33 & 12.02 & 37.75 & 89.50 \\ \bottomrule
\end{tabular*}
\end{table}

The \textit{boxplots} summarizes these results in \autoref{fig:bp-blob}.
Aside from the spread of the values regarding the variable answer and the outliers in the variable time, in general, the performance of the participants are better when the anti-pattern Blob is not present.

\begin{figure*}
% \centering
\begin{subfigure}{.2\linewidth}
    \includegraphics[width=1\linewidth]{boxplot-time-blob.pdf}
    \caption{Time spent.}
    \label{fig:bp-time-blob}
\end{subfigure}\hfill%
\begin{subfigure}{.2\linewidth}
    \includegraphics[width=1\linewidth]{boxplot-answer-blob.pdf}
    \caption{Correctness of Answers.}
    \label{fig:bp-answer-blob}
\end{subfigure}\hfill%
\begin{subfigure}{.2\linewidth}
    \centering
    \includegraphics[width=1\linewidth]{boxplot-effort-blob.pdf}
    \caption{Overall Effort.}
    \label{fig:bp-effort-blob}
\end{subfigure}
\caption{Boxplot of the exploratory analysis with three dependent variables (time, answer, and effort) and the Blob anti-pattern (treatment).}
\label{fig:bp-blob}
\end{figure*}

The \autoref{fig:bp-exp-blob} shows the \textit{boxplots} grouped by experiments. Although the experiments were made with the same setup and design, the results presented a clear gap in the values.
The Experiment \#3, with the tasks performed with the anti-pattern Blob, shows \emph{inferior performance} from the participants in all the variables (time, accuracy, and effort);
while in Experiment \#5, this difference is not evident.

\begin{figure}
% \centering
\begin{subfigure}{.5\textwidth}
    \includegraphics[width=1\linewidth]{boxplot-time-by-experiment-blob.pdf}
    \caption{Time spent.}
    \label{fig:bp-time-experiment-blob}
\end{subfigure}\hfill%
\begin{subfigure}{.5\textwidth}
    \includegraphics[width=1\linewidth]{boxplot-answer-by-experiment-blob.pdf}
    \caption{Correctness of Answers.}
    \label{fig:bp-answer-experiment-blob}
\end{subfigure}\hfill%
\begin{subfigure}{.5\textwidth}
    \includegraphics[width=1\linewidth]{boxplot-effort-by-experiment-blob.pdf}
    \caption{Overall Effort.}
    \label{fig:bp-effort-experiment-blob}
\end{subfigure}
\caption{Boxplot of the exploratory analysis with dependent variables and the Blob anti-pattern (treatment) grouped by experiments.}
\label{fig:bp-exp-blob}
\end{figure}

The \autoref{fig:vp-blob} shows the \textit{violin plot} with the skill level of each participant in \emph{Software Engineering}, \emph{Java}, and \emph{Eclipse}. These values were gathered in a post-mortem questionnaire (see Section~\ref{sec:method}).
The participants of the Experiment \#6 have lower skills level in Software Engineering and Eclipse but similar for Java.
This might show that there is a relationship between the expertise and the performance of the participants in tasks with anti-patterns. For example, in our case, the participants with better technical skills had better results with instances of code without Blob anti-pattern.

\begin{figure*}
% \centering
\begin{subfigure}{.2\textwidth}
    \includegraphics[width=1\linewidth]{violinplot-skills-blob-se.pdf}
    % \caption{Software Engineering Expertise.}
    \label{fig:vp-blob-se}
\end{subfigure}\hfill%
\begin{subfigure}{.2\textwidth}
    \includegraphics[width=1\linewidth]{violinplot-skills-blob-java.pdf}
    % \caption{Java Expertise.}
    \label{fig:vp-blob-java}
\end{subfigure}\hfill%
\begin{subfigure}{.2\textwidth}
    \centering
    \includegraphics[width=1\linewidth]{violinplot-skills-blob-eclipse.pdf}
    % \caption{Eclipse Engineering Expertise.}
    \label{fig:vp-blob-eclipse}
\end{subfigure}
\caption{Violin plot, for Experiments \#3 and \#5, with Blob anti-pattern, showing the distribution of participants' expertise level regarding their skills in \emph{Software Engineering}, \emph{Java}, and \emph{Eclipse}.}
\label{fig:vp-blob}
\end{figure*}

Before applying the \textit{LMM} analysis method, we assess the normality of the residuals with the \textit{Shapiro Test}, indicating that the data are normally distributed for any dependent variable. Moreover, the \textit{Mean of Residuals} is ``0'' for all dependent variables.

\autoref{tab:lmm-anova-blob} shows the results of the \textit{LMM} analysis method.
The variables \textit{treatment} (anti-pattern Blob), \textit{experiment} (Experiments \#3 and \#5), as well as their interaction (denoted as \textit{treat.:experiment} in \autoref{tab:lmm-anova-blob}) affect the time spent, correctness of answers and participants' effort (the p-values are less than $\alpha=0.05$). The variable \textit{object}, that is, the Java system used in the tasks, impact the correctness of the answers (while it does not impact the time spent and participants' effort). This observation could mean that some systems/tasks were more difficult to perform. Lastly, the interaction between \textit{treatment} and \textit{object} (denoted as \textit{treat.:object} in \autoref{tab:lmm-anova-blob}) affects the time spent (while the correctness of the answers and participants' effort are not affected).

\begin{table*}
\footnotesize
\caption{Output of the execution of the \textit{LMM} analysis method, \textit{Shapiro Test} and \textit{Mean of Residuals} for the Blob anti-pattern. Significant effects are displayed in bold.}
\label{tab:lmm-anova-blob}
\begin{tabular*}{\tblwidth}{@{}Lrrrrr|rr@{}}
\toprule
& Treat. & Experiment & Object & Treat.:Object & Treat.:Exp. & Shapiro & Res. \\ \midrule
Time & \textbf{\textless~0.01} & \textbf{0.03} & 0.59 & \textbf{0.03} & \textbf{\textless~0.01} & 0.52 & 0 \\
Answer & \textbf{\textless~0.01} & \textbf{\textless~0.01} & \textbf{ \textless~0.01} & 0.22 & \textbf{\textless~0.01} & 0.82 & 0 \\
Effort & \textbf{\textless~0.01} & \textbf{0.04} & 0.74 & 0.96 & \textbf{\textless~0.01} & 0.43 & 0 \\ \bottomrule
\end{tabular*}
\end{table*}

% \begin{tcolorbox}[width=\linewidth]
    \paragraph{Summary of Results (Blob):}
    The results of the \textit{descriptive statistics}, \textit{boxplots} and the \textit{LMM} analysis method show that the anti-pattern Blob, when present in a java source code, decreases the developers' productivity by increasing the time spent in the tasks, reducing the accuracy of the answers and increasing the necessary effort. Moreover, the effect of anti-pattern seems to be more clear with participants with better technical expertise.
% \end{tcolorbox}


==> sec-results-sc.tex <==
% !TeX root = text-main.tex
% !TeX spellcheck = en_US
% !TeX encoding = UTF-8%
\subsection{Results of the Experiments with the Spaghetti Code Anti-pattern}
\label{sec:results-sc}

This section presents the results of the experiments that use the Spaghetti Code anti-pattern. It presents the \textit{descriptive statistics} for each dependent variable together with the \textit{boxplots}. Subsequently, it shows the results of the \textit{LMM} analysis method.

\autoref{tab:ds-sc} reports the descriptive statistics regarding the
\emph{time} spent (in seconds) during the tasks, correctness of the
\emph{answers} (in percentage), and the \emph{effort} (in percentage) used to complete the tasks.
The tasks performed  on code containing the anti-pattern Spaghetti Code are, on average, \emph{39.50\% more time consuming} when compared to code without the anti-pattern.
The answers in the tasks containing the anti-pattern Spaghetti Code are, on average, \emph{25.30\% less accurate} when compared to task with code without the anti-pattern.
Finally, the participants reported, on average, using \emph{more effort (around 10\% more)} when performing tasks involving code that contained the anti-pattern Spaghetti Code.

\begin{table}
\footnotesize
\caption{Descriptive statistics showing the aggregated results for the anti-pattern \emph{Spaghetti Code}.}
\label{tab:ds-sc}
\centering
\begin{tabular*}{\tblwidth}{@{}Llrrrrr@{}}
\toprule
D.Var. & Treat. & \multicolumn{1}{l}{Mean} & \multicolumn{1}{l}{Median} & \multicolumn{1}{l}{SD} & \multicolumn{1}{l}{Min} & \multicolumn{1}{l}{Max} \\ \midrule
Time & - & 184.58 & 183.96 & 56.54 & 86.67 & 314.58 \\
Time & Spagh. & 257.50 & 253.83 & 74.61 & 119.92 & 457.67 \\ \addlinespace
Answer & - & 52.84 & 52.50 & 13.07 & 29.17 & 79.17 \\
Answer & Spagh. & 27.55 & 26.50 & 17.15 & 4.17 & 66.83 \\ \addlinespace
Effort & - & 55.67 & 56.50 & 10.36 & 35.50 & 74.75 \\
Effort & Spagh. & 65.46 & 64.21 & 11.98 & 41.50 & 89.58 \\ \bottomrule
\end{tabular*}
\end{table}

The \textit{boxplots} summarizes these results in \autoref{fig:bp-sc}.
Aside of the spread of the values regarding the variable answer, in general, the performance of the participants are better when the anti-pattern Spaghetti Code is not present.

\begin{figure*}
\begin{subfigure}{.2\textwidth}
    \includegraphics[width=1\linewidth]{boxplot-time-sc.pdf}
    \caption{Time spent.}
    \label{fig:bp-time-sc}
\end{subfigure}\hfill%
\begin{subfigure}{.2\textwidth}
    \includegraphics[width=1\linewidth]{boxplot-answer-sc.pdf}
    \caption{Correctness of Answers.}
    \label{fig:bp-answer-sc}
\end{subfigure}\hfill%
\begin{subfigure}{.2\textwidth}
    \centering
    \includegraphics[width=1\linewidth]{boxplot-effort-sc.pdf}
    \caption{Overall Effort.}
    \label{fig:bp-effort-sc}
\end{subfigure}
\caption{Boxplot of the exploratory analysis with three dependent variables (time, answer, and effort) and the Spaghetti Code anti-pattern (treatment).}
\label{fig:bp-sc}
\end{figure*}

\autoref{fig:bp-exp-sc} shows the \textit{boxplots} grouped by experiments. Although the experiments were made with the same setup and design, the outcome presents disparity in its values.
The Experiment \#4, with the tasks performed with the anti-pattern Spaghetti Code, shows \emph{inferior performance} from the participants in all the variables (time, accuracy, and effort);
while in the Experiment \#6, this difference is not clear. Also, for the variable effort, the results are slightly contradictory, by showing better results when the anti-pattern is present.

\begin{figure}
\centering
\begin{subfigure}{.5\textwidth}
    \includegraphics[width=1\linewidth]{boxplot-time-by-experiment-sc.pdf}
    \caption{Time spent.}
    \label{fig:bp-sc-time-experiment}
\end{subfigure}\hfill%
\begin{subfigure}{.5\textwidth}
    \includegraphics[width=1\linewidth]{boxplot-answer-by-experiment-sc.pdf}
    \caption{Correctness of Answers.}
    \label{fig:bp-sc-answer-experiment}
\end{subfigure}\hfill%
\begin{subfigure}{.5\textwidth}
    \includegraphics[width=1\linewidth]{boxplot-effort-by-experiment-sc.pdf}
    \caption{Overall Effort.}
    \label{fig:bp-sc-effort-experiment}
\end{subfigure}
\caption{Boxplot of the exploratory analysis with dependent variables and the Spaghetti Code anti-pattern (treatment) grouped by Experiment.}
\label{fig:bp-exp-sc}
\end{figure}

The \autoref{fig:vp-sc} shows the \textit{violin plot} with the skill level of each participant in \emph{Software Engineering}, \emph{Java}, and \emph{Eclipse}. These values were gathered in a post-mortem questionnaire (see Section~\ref{sec:method}).
The participants of the Experiment \#6 have lower skills level in Software Engineering and Eclipse but similar for Java.
This might show that there is a relationship between the expertise and the performance of the participants in tasks with anti-patterns. For example, in our case, the participants with better technical skills, especially in Software Engineering and Eclipse had better results with instances of code without Spaghetti Code anti-pattern.

\begin{figure}
\centering
\begin{subfigure}{.16\textwidth}
    \includegraphics[width=1\linewidth]{violinplot-skills-sc-se.pdf}
    % \caption{Software Engineering Expertise.}
    \label{fig:vp-sc-se}
\end{subfigure}\hfill%
\begin{subfigure}{.16\textwidth}
    \includegraphics[width=1\linewidth]{violinplot-skills-sc-java.pdf}
    % \caption{Java Expertise.}
    \label{fig:vp-sc-java}
\end{subfigure}\hfill%
\begin{subfigure}{.16\textwidth}
    \centering
    \includegraphics[width=1\linewidth]{violinplot-skills-sc-eclipse.pdf}
    % \caption{Eclipse Engineering Expertise.}
    \label{fig:vp-sc-eclipse}
\end{subfigure}
\caption{Violin plot, for Experiments \#4 and \#6, with Spaghetti Code anti-pattern, showing the distribution of participants' expertise level regarding their skills in \emph{Software Engineering}, \emph{Java}, and \emph{Eclipse}.}
\label{fig:vp-sc}
\end{figure}

Before applying the \textit{LMM} analysis method, we assessed the normality of the residuals with the \textit{Shapiro Test}. The variable \textit{answer} had a value less than 0.05, indicating non-normally distributed residuals (while the residuals for the other dependent variables were normally distributed).
Consequently, we could not apply the \textit{LMM} analysis method.
Therefore, we used the \textit{Friedman Test} for the variable answer\footnote{As suggested by the reviewers, we decided to keep the values from the LMM as its outcome is the same as the Friedman Test, that is, \emph{\textless~0.01}.}.
% For this reason, we could only analyze the effect of the independent variable \textit{treatment}.
 % As for the \textit{Mean of Residuals}, it is ``0'' for any dependent variable.



\autoref{tab:lmm-anova-sc} shows the results of the \textit{LMM} analysis method. The variable \textit{treatment} (anti-pattern Spaghetti Code) affects the time spent, correctness of answers, and participants' effort. We can also observe that the variable \textit{experiment} (Experiments \#4 and \#6) and the interaction between \textit{treatment} and \textit{experiment} affects the time spent (while the variable \textit{object} and its interaction with the variable \textit{treatment} do not affect the time spent). Lastly, the variable \textit{object}, that is, the Java system used in the tasks, impact the participants' effort as well as the interaction between the variable \textit{treatment} and \textit{experiment} (while \textit{experiment} and the interaction between \textit{treatment} and \textit{object} do not impact the participants' effort).

\begin{table*}
    \footnotesize
\caption{Output of the execution of the \textit{LMM} analysis method, \textit{Shapiro Test} and \textit{Mean of Residuals} for the Spaghetti Code anti-pattern. Significant effects are displayed in red.}
\label{tab:lmm-anova-sc}
\begin{tabular*}{\tblwidth}{@{}Lrrrrr|rr@{}}
\toprule
& Treat. & Experiment & Object & Treat.:Object & Treat.:Exp. & Shapiro & Res. \\ \midrule
Time & \textbf{\textless~0.01} & \textbf{\textless~0.01} & 0.79 & 0.74 & \textbf{\textless~0.01} & 0.11 & 0 \\
\rowcolor[HTML]{EFEFEF}
Answer & \textbf{\textless~0.01} & \textbf{\textless~0.01} & 0.41 & 0.66 & \textbf{\textless~0.01} & \textbf{ 0.02} & 0 \\
Effort & \textbf{\textless~0.01} & 0.08 & \textbf{\textless~0.01} & 0.64 & \textbf{\textless~0.01} & 0.49 & 0 \\ \bottomrule
\end{tabular*}
\end{table*}

% \begin{tcolorbox}[width=\linewidth]
    \paragraph{Summary of Results (Spaghetti Code):}
    The results of the \textit{descriptive statistics}, \textit{boxplots} and the \textit{LMM} analysis method show that the anti-pattern Spaghetti Code, when present in a java source code, decreases the productivity by increasing the time spent in the tasks, reducing the accuracy of the answers, and increasing the necessary effort.
    Moreover, the effect of anti-pattern seems to be more clear with participants with better technical expertise.
% \end{tcolorbox}

